Homological Description of the Quantum Adiabatic Evolution With a View Toward Quantum Computations

We import the tools of Morse theory to study quantum adiabatic evolution, the core mechanism in adiabatic quantum computations (AQC). AQC is computationally equivalent to the (pre-eminent paradigm) of the Gate model but less error-prone, so it is ideally suitable to practically tackle a large number of important applications. AQC remains, however, poorly understood theoretically and its mathematical underpinnings are yet to be satisfactorily identified. Through Morse theory, we bring a novel perspective that we expect will open the door for using such mathematics in the realm of quantum computations, providing a secure foundation for AQC. Here we show that the singular homology of a certain cobordism, which we construct from the given Hamiltonian, defines the adiabatic evolution. Our result is based on E. Witten's construction for Morse homology that was derived in the very different context of supersymmetric quantum mechanics. We investigate how such topological description, in conjunction with Gau\ss-Bonnet theorem and curvature based reformulation of Morse lemma, can be an obstruction to any computational advantage in AQC. We also explore Conley theory, for the sake of completeness, in advance of any known practical Hamiltonian of interest. We conclude with the instructive case of the ferromagnetic $p-$spin where we show that changing its first order quantum transition (QPT) into a second order QPT, by adding non-stoquastic couplings, amounts to homotopically deform the initial surface accompanied with birth of pairs of critical points. Their number reaches its maximum when the system is fully non-stoquastic. In parallel, the total Gaussian curvature gets redistributed (by the Gau\ss--Bonnet theorem) around the new neighbouring critical points, which weakens the severity of the QPT.

==> Homological Description of the Quantum Adiabatic EvolutionWith a View Toward Quantum Computations - Version 2 /macros.tex <==
% MACROS these R. Dridi
% ---------------------
% caligraphique
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calR}{{\cal R}}
\def\D{\mathcal{D}}
\def\L{\mathcal{L}}
\def\S{\mathcal{S}}
\def\I{\mathcal{I}}
\def\V{\mathcal{V}}
\def\E{\mathcal{E}}
\def\H{$(\mathcal{H})$}
% Ensemble de nombres
\newcommand{\N}{{\mathbb N}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\K}{{\mathbb K}}

\newcommand{\Frac}[2]{\displaystyle \frac{#1}{#2}}
\newcommand{\Sum}[2]{\displaystyle{\sum_{#1}^{#2}}}
\newcommand{\Prod}[2]{\displaystyle{\prod_{#1}^{#2}}}
\newcommand{\Int}[2]{\displaystyle{\int_{#1}^{#2}}}
\newcommand{\Lim}[1]{\displaystyle{\lim_{#1}\ }}

\newcommand{\DF}[4]{\Frac{\partial^2 f_{#1 #2}}{\partial u_{#3} \partial u_{#4}}}

\newcommand{\tab}{\hspace*{\fill}}
\newcommand{\bs}{{\backslash}}
\newcommand{\eps}{{\varepsilon}}
\newcommand{\into}{{\;\rightarrow\;}}
\def\Hat{\widehat}
\def\Bar{\overline}
\def\vect{\vec}
\def\fbar{{\bar f}}
\def\xbar{{\bar \x}}

\def\Maple{{\sc Maple}}
\def\RG{{\sc Rosenfeld-Gr\"obner}}
%\newcommand{\iff}{{\;\longleftrightarrow\;}}

%%%%%%  mathrm
\def \rank{\mathrm{rang}}
\def \ord{\mathrm{ord}}
\def \dim{\mathrm{dim}}
\def \aut{\mathrm{Aut}^{\mathrm{loc}} }
\def \Id{\mathrm{Id}}
\def \Hom{\mathrm{Hom}}
\def \span{\mathrm{span}}
\def \codim{\mathrm{codim}}
\def \Ker{\mathrm{ker}}
\def \coKer{\mathrm{coker}}
\def \diff{\mathrm{Diff}^{\mathrm{loc}} }
\def \diffg{\mathrm{Diff} }
\def \rp{\mathrm{rp}}
\def \card{\mathrm{card}}
\def \leader{\mathrm{ld}}
\def \Esc{\mathrm{Esc}}

\def\J{\mathrm{J}}
\def\x{\mathrm{x}}
\def\a{\mathrm{a}}
\def\d{\mathrm{d}}

%%%%% Groupes
\def\GL{\mathrm{GL}}
\def\det{\mathrm{det}}
\def\SL{\mathrm{SL}}
\def\PSL{\mathrm{PSL}}
\def\PGL{\mathrm{PGL}}
\def\O{\mathrm{O}}

%%% Algebres de Lie
\def\gl{\mathfrak{gl}}
\def\g{\mathfrak{g}}
\def\h{\mathfrak{h}}

\def\Bar{\widehat}
%\def\fbar{{\widehat{f}}}

\newenvironment{Abstract}%
        {\begin{small}\centerline{\bf Abstract} \begin{quote}}
        {\end{quote} \end{small}}

\newenvironment{iitemize}
    {\begin{list}%
      {--}%
      {\setlength{\parsep}{2.5pt}
       \setlength{\itemsep}{2.5pt}
       \setlength{\topsep}{0pt}
       \setlength{\partopsep}{0pt}
      }
    }
    {\end{list}}

%\newcounter{menumi}
%\newenvironment{menumerate}%
%    {\begin{list}%
%      {(\roman{menumi})}%
%      {\usecounter{menumi}%
%       \setlength{\parsep}{0pt}%
%       \setlength{\itemsep}{0pt}%
%       \setlength{\topsep}{0pt}%
%       \setlength{\partopsep}{5pt}%
%       \setlength{\labelwidth}{10pt}%
%       \setlength{\labelsep}{5pt}%
%       \setlength{\leftmargin}{\labelwidth + \labelsep}%
%      }%
%    }%
%    {\end{list}}

%\newcounter{menumi}
\newenvironment{menumerate}{%
    \renewcommand{\theenumi}{\roman{enumi}}% 
    \renewcommand{\labelenumi}{\rm(\theenumi)}%
    \begin{enumerate}} {\end{enumerate}}
 

    
\newcommand{\afaire}{$$\vdots$$ \begin{center} {\sc a faire ...} \end{center} $$\vdots$$ }

\newcommand{\pref}[1]{(\ref{#1})}

% systemes d'equations
%\newenvironment{system}[1][]%
%{\begin{eqnarray} #1 \left\{ \begin{array}{lll}}%
%{\end{array} \right. \end{eqnarray}}

\newenvironment{meqnarray}%
	{\begin{eqnarray}  \begin{array}{rcl}}%
	{\end{array}  \end{eqnarray}}

%\newenvironment{proof}{\par \noindent {\sc DÈmonstration.} }
%			{\hfill {\sc CQFD}  \par}
%\newenvironment{remark}{\par \noindent {\bf Remarque. }}
%			{\hfill $\blacksquare$ \par}
%\newenvironment{example}{\par \noindent {\bf Exemple. }}
		%	{\hfill $\blacksquare$ \par}[chapter]

\newenvironment{Pmatrix}
        {$ \left( \!\! \begin{array}{rr} } 
        {\end{array} \!\! \right) $}


%
%\newtheorem{definition}{DÈfinition}
%\newtheorem{theorem}{ThÈor\`eme}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{Lemme}
%\newtheorem{corollary}{Corollaire}
%\newtheorem{example}{Exemple}
%\newtheorem{remark}{Remarque}
%\newtheorem{proof}{DÈmonstration}[chapter]



%%%%% Abbreviations
\def\MGMG{M\times G \times \overline M \times \overline G}
\def\RM{\calR(M)}
\def\cRM{\calR^*(M)}
\def\GM{G \times M}
\def\MG{M \times G}

\def\lbar{\overline}
\def\S{\mathcal{S}}
\def\Bar{\widehat}
%\def\fbar{{\widehat{f}}}

\newcommand{\fleche}[3]{#1 \stackrel{#2}\longrightarrow #3}
\def\ssi{si et seulement si\ }

%%%% Algos
%\newcommand{\algf}{\sffamily}
%\newcommand{\FUNCTION}{{\algf fonction}}
%\newcommand{\BEGIN}{{\algf debut}}
%\newcommand{\END}{{\algf fin}}

%\newcommand{\IF}{{\algf si}\ \ \ \=\+}
%\newcommand{\THEN}{{\algf alors}\ }
%\newcommand{\ELSE}{\=\-\kill{\algf sino}\=\+{\algf n}}
%\newcommand{\ELIF}{{\algf sinon}\=\+{\algf si}\ }
%\newcommand{\FI}{\=\-\kill{\algf fin si}\ }
%\newcommand{\FOR}{{\algf pour}\ \=\+}
%\newcommand{\ENDFOR}{\=\-\kill{\algf fin pour}\ }
%\newcommand{\FROM}{{\algf de}\ }
%\newcommand{\TO}{{\algf \a`a}\ }
%\newcommand{\WHILE}{{\algf tq}\ \ \ \=\+}
%\newcommand{\ENDWHILE}{\=\-\kill{\algf fin tq}}
%\newcommand{\DO}{{\algf faire}\ }
%\newcommand{\OD}{{\algf od}}
%\newcommand{\RETURN}{{\algf retourner}}
%\newcommand{\INDENTER}{{\algf si} \=\+\kill}


\newcommand{\algf}{\sffamily}
\newcommand{\BEGIN}{{\algf begin}}
\newcommand{\END}{{\algf end}}
\newcommand{\IF}{{\algf if}}
\newcommand{\THEN}{{\algf then}}
\newcommand{\ELSE}{{\algf else}}
\newcommand{\ELIF}{{\algf elif}}
\newcommand{\FI}{{\algf fi}}
\newcommand{\WHILE}{{\algf while}}
\newcommand{\FOR}{{\algf for}}
\newcommand{\DO}{{\algf do}}
\newcommand{\OD}{{\algf od}}
\newcommand{\RETURN}{{\algf return}}
\newcommand{\PROCEDURE}{{\algf procedure}}
\newcommand{\FUNCTION}{{\algf function}}
\newcommand{\INDENTER}{{\algf si} \=\+\kill}




%% OpÈrateurs

\newcommand{\initial}{\mathop{\mathsf{init}}}
\newcommand{\separant}{\mathop{\mathsf{sep}}}
\newcommand{\rem}{\mathop{\mathsf{rem}}}
\newcommand{\quo}{\mathop{\mathsf{quo}}}
\newcommand{\pquo}{\mathop{\mathsf{pquo}}}
\newcommand{\lcoeff}{\mathop{\mathsf{lcoeff}}}
\newcommand{\mvar}{\mathop{\mathsf{mvar}}}
\newcommand{\ld}{\mathop{\mathrm{ld}}}
%\newcommand{\rank}{\mathrm{\mathsf{rank}}}
\newcommand{\prem}{\mathop{\mathsf{prem}}}
\newcommand{\remp}{\mathrel{\mathsf{partial\_rem}}}
\newcommand{\remf}{\mathrel{\mathsf{full\_rem}}}
\renewcommand{\gcd}{\mathop{\mathrm{gcd}}}
\renewcommand{\deg}{\mathop{\mathrm{deg}}}
%\newcommand{\ord}{\mathop{\mathrm{ord}}}
\newcommand{\pairs}{\mathop{\mathrm{pairs}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ideal}[1]{(#1)}
\newcommand{\cont}{\mathop{\mathrm{cont}}}
\newcommand{\pp}{\mathop{\mathrm{pp}}}
\newcommand{\pgcd}{\mathop{\mathrm{pgcd}}}
\newcommand{\ppmc}{\mathop{\mathrm{ppcm}}}
\newcommand{\init}{\mathop{\mathrm{initial}}}
\newcommand{\NF}{\mathop{\mathrm{NF}}}
\newcommand{\rang}{\mathop{\mathrm{rang}}}
%\newcommand{\card}{\mathop{\mbox{card}}}
\newcommand{\Fr}{\mathop{\mathrm{Fr}}}

\newcommand{\trdeg}{\mathop{\mathrm{tr~deg}}}
\newcommand{\kk}{{\mathrm k}}
